LISPR: An Options Framework for Policy Reuse with Reinforcement Learning

We propose a framework for transferring any existing policy from a potentially unknown source MDP to a target MDP. This framework (1) enables reuse in the target domain of any form of source policy, including classical controllers, heuristic policies, or deep neural network-based policies, (2) attains optimality under suitable theoretical conditions, and (3) guarantees improvement over the source policy in the target MDP. These are achieved by packaging the source policy as a black-box option in the target MDP and providing a theoretically grounded way to learn the option's initiation set through general value functions. Our approach facilitates the learning of new policies by (1) maximizing the target MDP reward with the help of the black-box option, and (2) returning the agent to states in the learned initiation set of the black-box option where it is already optimal. We show that these two variants are equivalent in performance under some conditions. Through a series of experiments in simulated environments, we demonstrate that our framework performs excellently in sparse reward problems given (sub-)optimal source policies and improves upon prior art in transfer methods such as continual learning and progressive networks, which lack our framework's desirable theoretical properties.

==> proofs_greward.tex <==
\subsection{Proxies for Recovery Rewards}

\todo[inline]{DG: This reference \citep{vecerik2019rewardestimation} is a special case of what we propose here and helps motivate it.  Their reward predictor is a special case of our success predictor (with gamma=0) and thus their prediction does not depend on a policy like our work.  The policy they learn maximizes the future accumulated reward predictor directly.  But they see benefits from sharing features in addition to using this to estimate the reward (without expensive hardware) - this is something we can explore in follow up work particularly with real-world experiments.}
\todo[inline]{We need to highlight the advantage offered by using G(s) as the reward in recovery policy learning - can make a sparse reward dense.  Can we depict an example of this?  One advantage is that the SP does not require an oracle reward since the G(s) can be used directly as the reward.}
\todo[inline]{DG: The GVF replaces the need for an oracle reward signal especially relavent in many manipulation tasks - cite \citep{vecerik2019rewardestimation}}
In this section, we show how the GVF $G(s)$ can be used in different ways to estimate the recovery policy reward to learn the recovery policy.  At first, it might be unclear why one might want to do this since one generally has access to the rewards of the target MDP which can be used to learn the value function of the recovery policy with Definition \ref{def_recovery_option}.  However, $G(s)$ learning can be decoupled from recovery policy learning since the source policy does not change; this can be advantageous in real-world tasks where collecting experience is expensive \citep{graves2020}.  For example, one approach to training a robot to successfully insert a peg into a hole is to train a reward predictor to identify succeed and failed insertions \citep{vecerik2019rewardestimation} and share those features with the policy.  Our success predictor in Definition \ref{def_success} is a generalization of the reward predictor in \citep{vecerik2019rewardestimation}.  Thus, there may be real-world benefits to using the success predictor to learn policies including (1) faster learning through sharing of features, and (2) eliminating the dependency on ad hoc reward shaping and additional hardware and sensors that provide rich reward signals for learning.

We define three possible rewards using only $G(s)$ and provide proofs on whether or not they are biased estimators of the recovery policy reward in Equation \eqref{eq_recovery_reward} are given in the appendix.  We also provide an example highlighting the power of the predictions.

\todo[inline]{This section is less important and can be moved to appendix probably.  However, it should be mentioned that this is different from potential-based reward shaping \citep{ng1999} which is $\gamma\phi(s')-\phi(s)$ since our method is $G(s,a) - \gamma G(s')$ where the sign is flipped and $G(s,a)$ is not only a function of state but also of action.}

\begin{restatable}{lem}{diffunbiasedtheorem}
Learning a recovery policy given in Definition \ref{def_recovery_option} where the recovery policy reward is replaced by $\hat{r}^{R}(s_t,a_t,s_{t+1})=G(s_t,a_t) - \zeta(s_{t+1})G(s_{t+1})$ results in the value function $\hat{V}^{R}(s_t)$ which is an unbiased estimate of the value function $V^{R}(s_t)$ for all states $s_t \in S$.
\label{lem_diff_unbiased_theorem}
\end{restatable}
\begin{restatable}{lem}{gbiasedtheorem}
Learning a recovery policy given in Definition \ref{def_student_option} where the recovery policy reward is replaced by $\hat{r}^{R}(s_t,a_t,s_{t+1})=(1-\zeta(s_{t+1}))G(s_t,a_t)$ results in the value function $\hat{V}^{R}(s_t)$ which is a biased estimate of the value function $V^{R}(s_t)$ for all states $s_t \in S$ with bias characterized by $(1-\gamma) \E_{R} \left[ \sum_{i=0}^{T-2}{\gamma^i G(s_{t+1})} - \gamma\sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} | s=s_t \right]$ for $0 \leq \gamma < 1$.
\label{lem_g_biased_theorem}
\end{restatable}

The bias characterized in Lemma \ref{lem_g_biased_theorem} is quite small for large values of $\gamma$; thus, we argue that the bias is negligible for most RL problems with large values of $\gamma$.  It should be noted however that in the limit as $\gamma \to 1$, the bias while small, is not eliminated in the general case.  If the reward of the target MDP is zero, i.e. $r_{t+1}, r_{t+2}, r_{t+T-1}$ are all zero, then in the limit as $\gamma \to 1$ the bias is eliminated.

\begin{restatable}{lem}{nextgbiasedtheorem}
Learning a recovery policy given in Definition \ref{def_student_option} where the recovery policy reward is replaced by $\hat{r}^{R}(s_t,a_t,s_{t+1})=(1-\zeta(s_{t+1}))G(s_{t+1})$ results in the value function $\hat{V}^{R}(s_t)$ which is a biased estimate of the value function $V^{R}(s_t)$ for all states $s_t \in S$ with bias characterized by $\E_{R} \left[(1-\gamma) \sum_{i=0}^{T-2}{ \gamma^i G(s_{t+1}) } - \sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} | s=s_t \right]$.
\label{lem_nextg_biased_theorem}
\end{restatable}

The bias characterized in Lemma \ref{lem_nextg_biased_theorem} could be substantial for some target MDP rewards.  If the reward of the target MDP is zero, i.e. $r_{t+1}, r_{t+2}, r_{t+T-1}$ are all zero, then in the limit as $\gamma \to 1$ the bias is eliminated.

\todo[inline]{The theory in this section might need some "help" - why do we need $(1-\gamma)$ terms?  Maybe we need to make some arguments about weak-stationarity?}
\todo[inline]{We need to add an example here of how using G(s) is denser than using just the reward if it is sparse}

% Additional material
% TODO: Do we need to prove that L is bigger than the set of terminal states that end in success?  This should be obvious but motivates why recovery policy can tolerate sparse cumulants. (ready)

\todo[inline]{We need more context for this - for now it sits in the appendix.  We can consider removing it}
It is tempting to define an alternative reward for the recovery policy where
\begin{equation}
    r^{R}_{t+1}=
    \begin{cases}
        1 & \text{ if $s_{t+1} \in L$}\\
        0 & \text{otherwise}
    \end{cases}
    \label{eq_sp_alternative_reward}
\end{equation}
for a given source policy with initiation set $L$.  It can be shown that the recovery policy does not maximize the future sum of rewards, i.e. $\sum_{i=0}^{\infty}{\gamma^i r_{t+i+1}}$, of the target MDP in the general case since the recovery policy ignores the value of $G(s)$ for states $s \in L$. However, under the condition that the target MDP reward is binary $r_t \in {0,1}$, the reward $r_t=1$ is given only on successful completion of the task and the discount of the success predictor is $\gamma=1$, then this alternative reward can be shown to be equivalent to \eqref{eq_recovery_reward}.

\subsection{Recovery Value Biases}
Here we characterize the biases in estimating the recovery policy value function $V^{R}(s)$ with the GVF $G(s)$.

\diffunbiasedtheorem*
\begin{proof}
Given a primal option in Definition \ref{def_primal_option} and a corresponding recovery option in Definition \ref{def_student_option}, let us define a value function $\hat{V}^{R}(s)$ with reward $\hat{r}^{R}(s_t,a_t,s_{t+1}) = G(s_t,a_t) - \gamma (1 - \beta(s_{t+1}))G(s_{t+1})$ where $\beta(s_{t+1})$ is given in Equation \eqref{eq_recovery_termination} for all $s_t \in S$, any action $a_t \in A$, and $s_{t+1} \sim P(s_{t+1}|s_t,a_t)$.  One can simplify the notation by defining a continuation function $\gamma(s)=\gamma (1 - \beta(s))$ such that $\hat{r}^{R}(s_t,a_t,s_{t+1}) = G(s_t,a_t) - \gamma(s_{t+1})G(s_{t+1})$.

First, we will define $\tilde{r}_t=G(s_t,a_t) - \gamma G(s_{t+1})$ and show that it reduces to the expected $r_t$ in the target MDP for all transitions $s_t \in S$, any action $a_t \in A$, and $s_{t+1} \sim P(s_{t+1}|s_t,a_t)$.
\begin{equation}
    \begin{split}
        \tilde{r}_t & = G(s_t,a_t) - \gamma G(s_{t+1}) \\
            & = \E_{\mu} \left[ \sum_{i=0}^{\infty}{\gamma^i r_{t+i+1}} | s_t,a_t \right] - \gamma G(s_{t+1}) \\
            & = \E_{s_{t+1} \sim P} \left[ r_{t+1} | s_t,a_t \right] + \gamma G(s_{t+1}) - \gamma G(s_{t+1}) \\
            & = \E_{s_{t+1} \sim P} \left[ r_{t+1} | s_t,a_t \right]
    \end{split}
    \label{eq_recovery_reward_diff}
\end{equation}
Now, we can compute $\hat{V}^{R}(s)$ for all states $s \in S$.
\begin{equation}
    \begin{split}
        \hat{V}^{R}(s) = & \E_{R} \left[ \sum_{i=0}^{\infty}{ \left(  \prod_{j=0}^{i-1}{ \gamma_{t+j+1}} \right) r^{R}_{t+i+1}} | s=s_t \right] \\
                             = & \E_{R} \left[ \sum_{i=0}^{\infty}{ \left(                   \prod_{j=0}^{i-1}{\gamma_{t+j+1}} \right) \left( G(s_t,a_t) - \gamma_{t+1} G(s_{t+1}) \right)} | s=s_t \right] \\
                             = & \E_{R} \left[ \sum_{i=0}^{T-2}{ \gamma^i r_{t+i+1}} | s=s_t \right] + \gamma^{T-1} \E_{\mu} \left[\sum_{j=0}^{\infty}{\gamma^j r_{t+j+T}} | s_{T-1} \right] \\
                             = & V^{R}(s) \text{ (by Definition \ref{def_student_option})}
    \end{split}
\end{equation}
\end{proof}


\gbiasedtheorem*
\begin{proof}
The value function $\hat{V}^{R}(s)$ with reward $r^{R}_{t+1}=(1 - \gamma(s_{t+1}))G(s_t,a_t)$ for all states $s \in S$ is
\begin{equation}
    \begin{split}
        \hat{V}^{R}(s) = & \E_{R} \left[ \sum_{i=0}^{\infty}{ \left(  \prod_{j=0}^{i-1}{\gamma_{t+j+1}} \right) r^{R}_{t+i+1}} | s=s_t \right] \\
                             = & \E_{R} \left[ \sum_{i=0}^{\infty}{ \left(  \prod_{j=0}^{i-1}{\gamma_{t+j+1}} \right) \left( (1-\gamma(s_{t+1})) G(s_t,a_t) \right) } | s=s_t \right] \\
                             = & (1-\gamma) \E_{R} \left[ \sum_{i=0}^{T-2}{\gamma^i G(s_t, a_t)} |s=s_t \right] + \gamma^{T-1} G(s_{T-1},a_{T-1}) \\
                             = & (1-\gamma) \E_{R} \left[ \sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} + \sum_{i=0}^{T-2}{\gamma^i G(s_{t+1})} + \gamma^{T-1} \frac{G(s_{T-1},a_{T-1})}{1-\gamma} | s=s_t \right] \\
                             = & (1-\gamma) \E_{R} \left[ \frac{1-\gamma}{1-\gamma} \sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} + \sum_{i=0}^{T-2}{\gamma^i G(s_{t+1})} + \gamma^{T-1} \frac{G(s_{T-1},a_{T-1})}{1-\gamma} | s=s_t \right] \\
                             = & (1-\gamma) \E_{R} \left[ \frac{V^{R}(s_t)}{1-\gamma} + \sum_{i=0}^{T-2}{\gamma^i G(s_{t+1})} - \gamma\sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} | s=s_t \right] \\
                             = & V^{R}(s) + (1-\gamma) \E_{R} \left[ \sum_{i=0}^{T-2}{\gamma^i G(s_{t+1})} - \gamma\sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} | s=s_t \right] \\
    \end{split}
\end{equation}
Thus the bias is characterized by $(1-\gamma) \E_{R} \left[ \sum_{i=0}^{T-2}{\gamma^i G(s_{t+1})} - \gamma\sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} | s=s_t \right]$.
\end{proof}

\nextgbiasedtheorem*
\begin{proof}
The value function $\hat{V}^{R}(s)$ with reward $r^{R}_{t+1}=(1-\gamma(s_{t+1}))G(s_{t+1})$ for all states $s \in S$ is
\begin{equation}
    \begin{split}
        \hat{V}^{R}(s) = & \E_{R} \left[ \sum_{i=0}^{\infty}{ \left(  \prod_{j=0}^{i-1}{\gamma_{t+j+1}} \right) r^{R}_{t+i+1}} | s=s_t \right] \\
                             = & \E_{R} \left[ \sum_{i=0}^{\infty}{ \left(  \prod_{j=0}^{i-1}{\gamma_{t+j+1}} \right) (1-\gamma(s_{t+1})) G(s_{t+1}) } | s=s_t \right] \\
                             = & (1-\gamma) \E_{R} \left[ \sum_{i=0}^{T-2}{ \gamma^i G(s_{t+1}) } | s=s_t \right] + \gamma^{T-1} G(s_{T}) \\
                             = & V^{R}(s) + \E_{R} \left[(1-\gamma) \sum_{i=0}^{T-2}{ \gamma^i G(s_{t+1}) } - \sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} | s=s_t \right] \\
    \end{split}
\end{equation}
Thus the bias is characterized by $\E_{R} \left[(1-\gamma) \sum_{i=0}^{T-2}{ \gamma^i G(s_{t+1}) } - \sum_{i=0}^{T-2}{\gamma^i r_{t+i+1}} | s=s_t \right]$.
\end{proof}
